DiffPrompter: Differentiable Implicit Visual Prompts for Semantic-Segmentation in Adverse Conditions

Semantic segmentation in adverse weather scenarios is a critical task for autonomous driving systems. While foundation models have shown promise, the need for specialized adaptors becomes evident for handling more challenging scenarios. We introduce DiffPrompter, a novel differentiable visual and latent prompting mechanism aimed at expanding the learning capabilities of existing adaptors in foundation models. Our proposed $\nabla$HFC image processing block excels particularly in adverse weather conditions, where conventional methods often fall short. Furthermore, we investigate the advantages of jointly training visual and latent prompts, demonstrating that this combined approach significantly enhances performance in out-of-distribution scenarios. Our differentiable visual prompts leverage parallel and series architectures to generate prompts, effectively improving object segmentation tasks in adverse conditions. Through a comprehensive series of experiments and evaluations, we provide empirical evidence to support the efficacy of our approach. Project page at https://diffprompter.github.io.

==> dummy/dummy.tex <==
\subsection{Quantitative Analysis:}
Here, we compare the quantitative results on 3 datasets namely VOCNormal Test set (V\_N\_Ts), VOCFoggy Test set (V\_F\_Ts) and real-world RTTS dataset for the foggy setting. 
We set the baseline as YoloV3 which is trained on hybrid data of foggy and clear images to validate if we could improve the performance by only using data augmentation or not. We compare our results with domain adaption-based (DA-Yolo), multi-task learning-based (DSNet), defogging as pre-processing (MSBDN, GridDehaze) and adaptive image (IA-Yolo) methods.
